On The Expressivity of Objective-Specification Formalisms in Reinforcement Learning

Most algorithms in reinforcement learning (RL) require that the objective is formalised with a Markovian reward function. However, it is well-known that certain tasks cannot be expressed by means of an objective in the Markov rewards formalism, motivating the study of alternative objective-specification formalisms in RL such as Linear Temporal Logic and Multi-Objective Reinforcement Learning. To date, there has not yet been any thorough analysis of how these formalisms relate to each other in terms of their expressivity. We fill this gap in the existing literature by providing a comprehensive comparison of 17 salient objective-specification formalisms. We place these formalisms in a preorder based on their expressive power, and present this preorder as a Hasse diagram. We find a variety of limitations for the different formalisms, and argue that no formalism is both dominantly expressive and straightforward to optimise with current techniques. For example, we prove that each of Regularised RL, (Outer) Nonlinear Markov Rewards, Reward Machines, Linear Temporal Logic, and Limit Average Rewards can express a task that the others cannot. The significance of our results is twofold. First, we identify important expressivity limitations to consider when specifying objectives for policy optimization. Second, our results highlight the need for future research which adapts reward learning to work with a greater variety of formalisms, since many existing reward learning methods assume that the desired objective takes a Markovian form. Our work contributes towards a more cohesive understanding of the costs and benefits of different RL objective-specification formalisms.

==> figures/def-table.tex <==
\newcommand{\specialcell}[2][c]{%
  \begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
% t = top
% c = centre
% b = bottom


\begin{table}[t]
\centering
\begin{tabular}{|p{1.5cm}|p{1cm}|p{1cm}|p{3cm}|p{6cm}|p{1cm}|}
\hline
Formalism & Label & Tuple & Types & $\pi_1 \preceq_{E,O} \pi_2$ & Citation \\
\hline
\hline




% Name
Markovian Rewards & 
% Label
$MR$ &
% Tuple
$\langle R, \gamma \rangle$ &
% Type
$R: S \times A \times S \to \mathbb{R}$, $\gamma \in [0,1]$ &
% preceq
\specialcell[t]{
$J(\pi_1) \leq J(\pi_2)$ \\
$J(\pi) = \mathbb{E}[\sum_{t=0}^{\infty}(\gamma^t R(s_t, a_t, s_{t+1}))]$
} &
% Citation
\cite{sutton_and_barto} \\
\hline




% Name
XXX & 
% Label
$LAR$ &
% Tuple
$\langle \rangle$ &
% Type

% preceq
\specialcell[t]{

} &
% Citation
\cite{xxx} \\
\hline




% Name
XXX & 
% Label
$LTL$ &
% Tuple
$\langle \rangle$ &
% Type

% preceq
\specialcell[t]{

} &
% Citation
\cite{xxx} \\
\hline




% Name
XXX & 
% Label
$RM$ &
% Tuple
$\langle \rangle$ &
% Type

% preceq
\specialcell[t]{

} &
% Citation
\cite{xxx} \\
\hline




% Name
XXX & 
% Label
$CRL$ &
% Tuple
$\langle \rangle$ &
% Type

% preceq
\specialcell[t]{

} &
% Citation
\cite{xxx} \\
\hline




% Name
XXX & 
% Label
$INMR$ &
% Tuple
$\langle \rangle$ &
% Type

% preceq
\specialcell[t]{

} &
% Citation
\cite{xxx} \\
\hline




% Name
XXX & 
% Label
$IMORL$ &
% Tuple
$\langle \rangle$ &
% Type

% preceq
\specialcell[t]{

} &
% Citation
\cite{xxx} \\
\hline




% Name
XXX & 
% Label
$ONMR$ &
% Tuple
$\langle \rangle$ &
% Type

% preceq
\specialcell[t]{

} &
% Citation
\cite{xxx} \\
\hline




% Name
XXX & 
% Label
$OMORL$ &
% Tuple
$\langle \rangle$ &
% Type

% preceq
\specialcell[t]{

} &
% Citation
\cite{xxx} \\
\hline




% Name
XXX & 
% Label
$GOMORL$ &
% Tuple
$\langle \rangle$ &
% Type

% preceq
\specialcell[t]{

} &
% Citation
\cite{xxx} \\
\hline




% Name
XXX & 
% Label
$FTR$ &
% Tuple
$\langle \rangle$ &
% Type

% preceq
\specialcell[t]{

} &
% Citation
\cite{xxx} \\
\hline




% Name
XXX & 
% Label
$FTLR$ &
% Tuple
$\langle \rangle$ &
% Type

% preceq
\specialcell[t]{

} &
% Citation
\cite{xxx} \\
\hline




% Name
XXX & 
% Label
$FPR$ &
% Tuple
$\langle \rangle$ &
% Type

% preceq
\specialcell[t]{

} &
% Citation
\cite{xxx} \\
\hline




% Name
XXX & 
% Label
$X$ &
% Tuple
$\langle \rangle$ &
% Type

% preceq
\specialcell[t]{

} &
% Citation
\cite{xxx} \\
\hline

\end{tabular}
\caption{The definitions for each of the objective formalisms, their objective specifications, and the policy orderings those specifications induce}
\end{table}

==> figures/fig1-cat.tex <==
\begin{figure}[h]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \begin{tikzpicture}
            % Body
      \fill[gray!50] (0,0) circle (1);
      
      % Ears
      \fill[gray!50] (-0.7,0.7) -- (0,1.3) -- (0.7,0.7) -- cycle;
      \fill[gray!50] (-0.7,0.7) arc (180:360:0.7cm and 0.2cm);
      
      % Face
      \fill[white] (0,0) circle (0.8);
      
      % Eyes
      \fill[black] (-0.3,0.3) circle (0.1);
      \fill[black] (0.3,0.3) circle (0.1);
      
      % Nose
      \fill[black] (0,0) circle (0.05);
      
      % Whiskers
      \draw[black, thick] (-0.4,0) -- (-1.5,0);
      \draw[black, thick] (0.4,0) -- (1.5,0);
      \draw[black, thick] (-0.4,-0.2) -- (-1.5,-1);
      \draw[black, thick] (0.4,-0.2) -- (1.5,-1);
      \draw[black, thick] (-0.4,0.2) -- (-1.5,1);
      \draw[black, thick] (0.4,0.2) -- (1.5,1);
      
      % Whiskers reflection
      \draw[white, thick] (-0.4,-0.05) -- (-1.5,0.7);
      \draw[white, thick] (0.4,-0.05) -- (1.5,0.7);
      \draw[white, thick] (-0.4,0.15) -- (-1.5,-0.7);
      \draw[white, thick] (0.4,0.15) -- (1.5,-0.7);
      
      % Mouth
      \draw[black, thick] (-0.3,-0.4) .. controls (0,-0.8) .. (0.3,-0.4);
      
      % Whiskers reflection
      \draw[white, thick] (-0.3,-0.35) .. controls (0,-0.75) .. (0.3,-0.35);
      
    \end{tikzpicture}
    \caption{ChatGPT 3.5 is \emph{okay} at drawing a cat using the tikz package.}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \centering
    \begin{tikzpicture}
          % Draw the body
    \draw[fill=gray!50] (2,1) ellipse (1cm and 2cm);
    % Draw the head
    \draw[fill=gray!50] (4,2) ellipse (0.8cm and 1cm);
    % Draw the eyes
    \fill[white] (3.7,2.2) circle (0.15cm);
    \fill[white] (4.3,2.2) circle (0.15cm);
    % Draw the nose
    \fill[pink] (4,1.9) circle (0.07cm);
    % Draw the ears
    \draw[fill=gray!50] (3.2,2.8) -- (3.6,2.7) -- (3.4,2.5) -- cycle;
    \draw[fill=gray!50] (4.4,2.8) -- (4.0,2.7) -- (4.2,2.5) -- cycle;
    % Draw the tail
    \draw[thick, gray!50] (1.0,1.5) to [bend right=20] (0.2,2.0);
    % Draw the legs
    \draw[thick, gray!50] (2.3, 0) -- ++(0, -0.7);
    \draw[thick, gray!50] (1.7, 0) -- ++(0, -0.7);
    % Draw the whiskers
    \draw (4.1,1.8) -- ++(0.5,-0.1);
    \draw (4.1,1.85) -- ++(0.5,0);
    \draw (4.1,1.9) -- ++(0.5,0.1);
    \draw (3.9,1.8) -- ++(-0.5,-0.1);
    \draw (3.9,1.85) -- ++(-0.5,0);
    \draw (3.9,1.9) -- ++(-0.5,0.1);
    \end{tikzpicture}
    \caption{ChatGPT 4 draws a more detailed image, that is only slightly harrowing.}
  \end{subfigure}
  \caption{Note that, though neither drawing is good, both are much better than I could do.}
\end{figure}

==> gubbins/baseline.tex <==
\section{Baseline}

\subsection{MR vs Nonlinear MR (treating policies as functions from states to distributions over actions}
Claim: MR $\subset$ NMR. \\
Proof:\\
Definitions:\\
$\indent$1. NMR: $\pi_1 \prec \pi_2 \iff f(J(\pi_1)) < f(J(\pi_2))$\\
$\indent$2. MR: $\pi_1 \prec \pi_2 \iff J(\pi_1) < J(\pi_2)$\\
$\indent$3. $J(\pi) := \mathop{\mathbb{E}}_{s_0 \sim \mu_0}[V^\pi(s_0)]$\\
$\indent$4. $V^\pi(s) := \mathop{\mathbb{E}}_{a \sim \pi(s)}[\mathop{\mathbb{E}}_{s' \sim T(s,a)}[R(s,a) + \gamma V^\pi(s')]]$\\\\
Trivially, any policy ordering inducable with MR is also inducable with NMR. For an MDP (S,A,T,I,R,$\gamma$), the nonlinear MDP (NMDP) (S,A,T,I,R,$\gamma$,f), where f is the identity function on the reals, induces the same policy ordering.

\subsection{MR vs Reward Machines}
A reward machine is defined as
$R_{PSA}=\langle U, u_0, \delta_u, \delta_r \rangle$ where \\
$U: \{u_0, u_1, ... u_n\}$\\
where $u_i$ are states in the machine and \\
$u_0 \in U$ \\
is the starting state \\
$\delta_u: U \times 2^P \rightarrow U$ \\
is the transition function \\
$\delta_r: U \times U \rightarrow [S \times A \times S \rightarrow \mathbb{R}]$
\\

Claim: MR $\subset$ RM. \\
Proof:
Given MR defined by $R$, define a reward machine 
$R_{PSA}=\langle {0}, 0, f(*) = 0, R \rangle$ \\
Trivially, any policy ordering inducable with the MR is also inducable with the RM.


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


==> write-up-sections/Appendices/app-definititions.tex <==
\section{Appendix: Definitions}

\begin{definition}
    
\end{definition}
